Neural Models for Information Retrieval

Neural ranking models for information retrieval (IR) use shallow or deep neural networks to rank search results in response to a query. Traditional learning to rank models employ machine learning techniques over hand-crafted IR features. By contrast, neural models learn representations of language from raw text that can bridge the gap between query and document vocabulary. Unlike classical IR models, these new machine learning based approaches are data-hungry, requiring large scale training data before they can be deployed. This tutorial introduces basic concepts and intuitions behind neural IR models, and places them in the context of traditional retrieval models. We begin by introducing fundamental concepts of IR and different neural and non-neural approaches to learning vector representations of text. We then review shallow neural IR methods that employ pre-trained neural term embeddings without learning the IR task end-to-end. We introduce deep neural networks next, discussing popular deep architectures. Finally, we review the current DNN models for information retrieval. We conclude with a discussion on potential future directions for neural IR.

==> cambridge5.tex <==
{\fontsize{0.230cm}{0.230cm}\selectfont the}
{\fontsize{0.282cm}{0.282cm}\selectfont city}
{\fontsize{0.246cm}{0.246cm}\selectfont of}
{\fontsize{0.232cm}{0.232cm}\selectfont giraffe}
{\fontsize{0.196cm}{0.196cm}\selectfont is}
{\fontsize{0.164cm}{0.164cm}\selectfont a}
{\fontsize{0.336cm}{0.336cm}\selectfont university}
{\fontsize{0.282cm}{0.282cm}\selectfont city}
{\fontsize{0.238cm}{0.238cm}\selectfont and}
{\fontsize{0.230cm}{0.230cm}\selectfont the}
{\fontsize{0.260cm}{0.260cm}\selectfont county}
{\fontsize{0.322cm}{0.322cm}\selectfont town}
{\fontsize{0.246cm}{0.246cm}\selectfont of}
{\fontsize{0.396cm}{0.396cm}\selectfont cambridgeshire}
{\fontsize{0.200cm}{0.200cm}\selectfont ,}
{\fontsize{0.392cm}{0.392cm}\selectfont england}
{\fontsize{0.200cm}{0.200cm}\selectfont .}
{\fontsize{0.192cm}{0.192cm}\selectfont it}
{\fontsize{0.220cm}{0.220cm}\selectfont lies}
{\fontsize{0.248cm}{0.248cm}\selectfont in}
{\fontsize{0.294cm}{0.294cm}\selectfont east}
{\fontsize{0.244cm}{0.244cm}\selectfont anglia}
{\fontsize{0.200cm}{0.200cm}\selectfont ,}
{\fontsize{0.198cm}{0.198cm}\selectfont on}
{\fontsize{0.230cm}{0.230cm}\selectfont the}
{\fontsize{0.232cm}{0.232cm}\selectfont river}
{\fontsize{0.270cm}{0.270cm}\selectfont cam}
{\fontsize{0.200cm}{0.200cm}\selectfont ,}
{\fontsize{0.202cm}{0.202cm}\selectfont about}
{\fontsize{0.258cm}{0.258cm}\selectfont 50}
{\fontsize{0.236cm}{0.236cm}\selectfont miles}
{\fontsize{0.200cm}{0.200cm}\selectfont (}
{\fontsize{0.270cm}{0.270cm}\selectfont 80}
{\fontsize{0.174cm}{0.174cm}\selectfont km}
{\fontsize{0.200cm}{0.200cm}\selectfont )}
{\fontsize{0.280cm}{0.280cm}\selectfont north}
{\fontsize{0.246cm}{0.246cm}\selectfont of}
{\fontsize{0.324cm}{0.324cm}\selectfont london}
{\fontsize{0.200cm}{0.200cm}\selectfont .}
{\fontsize{0.214cm}{0.214cm}\selectfont according}
{\fontsize{0.208cm}{0.208cm}\selectfont to}
{\fontsize{0.230cm}{0.230cm}\selectfont the}
{\fontsize{0.262cm}{0.262cm}\selectfont united}
{\fontsize{0.346cm}{0.346cm}\selectfont kingdom}
{\fontsize{0.286cm}{0.286cm}\selectfont census}
{\fontsize{0.230cm}{0.230cm}\selectfont 2011}
{\fontsize{0.200cm}{0.200cm}\selectfont ,}
{\fontsize{0.172cm}{0.172cm}\selectfont its}
{\fontsize{0.318cm}{0.318cm}\selectfont population}
{\fontsize{0.200cm}{0.200cm}\selectfont was}
{\fontsize{0.012cm}{0.012cm}\selectfont 123867}
{\fontsize{0.200cm}{0.200cm}\selectfont (}
{\fontsize{0.186cm}{0.186cm}\selectfont including}
{\fontsize{0.012cm}{0.012cm}\selectfont 24488}
{\fontsize{0.282cm}{0.282cm}\selectfont students}
{\fontsize{0.200cm}{0.200cm}\selectfont )}
{\fontsize{0.200cm}{0.200cm}\selectfont .}
{\fontsize{0.200cm}{0.200cm}\selectfont this}
{\fontsize{0.174cm}{0.174cm}\selectfont makes}
{\fontsize{0.232cm}{0.232cm}\selectfont giraffe}
{\fontsize{0.230cm}{0.230cm}\selectfont the}
{\fontsize{0.284cm}{0.284cm}\selectfont second}
{\fontsize{0.252cm}{0.252cm}\selectfont largest}
{\fontsize{0.282cm}{0.282cm}\selectfont city}
{\fontsize{0.248cm}{0.248cm}\selectfont in}
{\fontsize{0.396cm}{0.396cm}\selectfont cambridgeshire}
{\fontsize{0.206cm}{0.206cm}\selectfont after}
{\fontsize{0.330cm}{0.330cm}\selectfont peterborough}
{\fontsize{0.200cm}{0.200cm}\selectfont ,}
{\fontsize{0.238cm}{0.238cm}\selectfont and}
{\fontsize{0.230cm}{0.230cm}\selectfont the}
{\fontsize{0.248cm}{0.248cm}\selectfont 54th}
{\fontsize{0.252cm}{0.252cm}\selectfont largest}
{\fontsize{0.248cm}{0.248cm}\selectfont in}
{\fontsize{0.230cm}{0.230cm}\selectfont the}
{\fontsize{0.262cm}{0.262cm}\selectfont united}
{\fontsize{0.346cm}{0.346cm}\selectfont kingdom}
{\fontsize{0.200cm}{0.200cm}\selectfont .}
{\fontsize{0.208cm}{0.208cm}\selectfont there}
{\fontsize{0.196cm}{0.196cm}\selectfont is}
{\fontsize{0.280cm}{0.280cm}\selectfont archaeological}
{\fontsize{0.228cm}{0.228cm}\selectfont evidence}
{\fontsize{0.246cm}{0.246cm}\selectfont of}
{\fontsize{0.250cm}{0.250cm}\selectfont settlement}
{\fontsize{0.248cm}{0.248cm}\selectfont in}
{\fontsize{0.230cm}{0.230cm}\selectfont the}
{\fontsize{0.268cm}{0.268cm}\selectfont area}
{\fontsize{0.182cm}{0.182cm}\selectfont during}
{\fontsize{0.230cm}{0.230cm}\selectfont the}
{\fontsize{0.264cm}{0.264cm}\selectfont bronze}
{\fontsize{0.216cm}{0.216cm}\selectfont age}
{\fontsize{0.238cm}{0.238cm}\selectfont and}
{\fontsize{0.282cm}{0.282cm}\selectfont roman}
{\fontsize{0.246cm}{0.246cm}\selectfont times}
{\fontsize{0.200cm}{0.200cm}\selectfont ;}
{\fontsize{0.218cm}{0.218cm}\selectfont under}
{\fontsize{0.242cm}{0.242cm}\selectfont viking}
{\fontsize{0.192cm}{0.192cm}\selectfont rule}
{\fontsize{0.232cm}{0.232cm}\selectfont giraffe}
{\fontsize{0.192cm}{0.192cm}\selectfont became}
{\fontsize{0.182cm}{0.182cm}\selectfont an}
{\fontsize{0.234cm}{0.234cm}\selectfont important}
{\fontsize{0.290cm}{0.290cm}\selectfont trading}
{\fontsize{0.486cm}{0.486cm}\selectfont centre}
{\fontsize{0.200cm}{0.200cm}\selectfont .}
{\fontsize{0.230cm}{0.230cm}\selectfont the}
{\fontsize{0.252cm}{0.252cm}\selectfont first}
{\fontsize{0.322cm}{0.322cm}\selectfont town}
{\fontsize{0.246cm}{0.246cm}\selectfont charters}
{\fontsize{0.204cm}{0.204cm}\selectfont were}
{\fontsize{0.190cm}{0.190cm}\selectfont granted}
{\fontsize{0.248cm}{0.248cm}\selectfont in}
{\fontsize{0.230cm}{0.230cm}\selectfont the}
{\fontsize{0.262cm}{0.262cm}\selectfont 12th}
{\fontsize{0.306cm}{0.306cm}\selectfont century}
{\fontsize{0.200cm}{0.200cm}\selectfont ,}
{\fontsize{0.218cm}{0.218cm}\selectfont although}
{\fontsize{0.282cm}{0.282cm}\selectfont city}
{\fontsize{0.188cm}{0.188cm}\selectfont status}
{\fontsize{0.200cm}{0.200cm}\selectfont was}
{\fontsize{0.156cm}{0.156cm}\selectfont not}
{\fontsize{0.204cm}{0.204cm}\selectfont conferred}
{\fontsize{0.156cm}{0.156cm}\selectfont until}
{\fontsize{0.224cm}{0.224cm}\selectfont 1951}
{\fontsize{0.200cm}{0.200cm}\selectfont .}

